SystemC Model of Power Side-Channel Attacks Against AI Accelerators: Superstition or not?

As training artificial intelligence (AI) models is a lengthy and hence costly process, leakage of such a model's internal parameters is highly undesirable. In the case of AI accelerators, side-channel information leakage opens up the threat scenario of extracting the internal secrets of pre-trained models. Therefore, sufficiently elaborate methods for design verification as well as fault and security evaluation at the electronic system level are in demand. In this paper, we propose estimating information leakage from the early design steps of AI accelerators to aid in a more robust architectural design. We first introduce the threat scenario before diving into SystemC as a standard method for early design evaluation and how this can be applied to threat modeling. We present two successful side-channel attack methods executed via SystemC-based power modeling: correlation power analysis and template attack, both leading to total information leakage. The presented models are verified against an industry-standard netlist-level power estimation to prove general feasibility and determine accuracy. Consequently, we explore the impact of additive noise in our simulation to establish indicators for early threat evaluation. The presented approach is again validated via a model-vs-netlist comparison, showing high accuracy of the achieved results. This work hence is a solid step towards fast attack deployment and, subsequently, the design of attack-resilient AI accelerators.

==> 07-Noise.tex <==
\section{Security Analysis and Evaluation}

\label{SecurityEvaluationSection}
In this section, we analyse the impact of noise on both the CPA and the Template attack and
%Consequently, we 
investigate the limits of such attacks based on the proposed SystemC model.

\subsection{Impact of Additive Noise on CPA}
\label{sec:cpa-additive-noise}
In applied cryptography, analysing the impact of additive noise on power attacks is essential \cite{lerm17cons} \cite{st09uni}.
The backbone of such an analysis is the leaked information's signal-to-noise ratio (SNR) \cite{bir16CPA}.
Here, additive noise is used and
the measurement noise is modelled by adding random values \(R_{n}\) with an average \(\bar{R}=0\) to the power trace \(P_{n}\) at each estimation point as  \(P_{n}+R_{n}\).
It can be gradually increased to have a bigger impact on the power estimation value and
%Here, 
we can set a fixed SNR to produce noisy power traces.
In order to statistically analyze the impact of the additive noise, the modified correlation coefficient \(\rho ^{\prime}(b_{k}) \) can be written as follows \cite{7951799}: 
\begin{equation}
\label{eq:correlation_noise1}
\resizebox{0.85\hsize}{!}{%
$\rho^{\prime} \left(b_{k}\right)=\frac{\sum_{n=0}^{N-1}\left(P_{n}+R_{n} -\bar{P}\right)\left(\hat{H}_{n, b_{k}}- \bar{H}_{b_{k}}\right)}{\sqrt{\sum_{n=0}^{N-1}\left(P_{n}+R_{n}-\bar{P}\right)^{2}} \sqrt{\Sigma_{n=0}^{N-1}\left( \hat{H_{n, b_{k}}}-\overline{H}_{n, b_{k}}\right)^{2}}}$}
\end{equation}


The additive random noise and Hamming distance variables are independent. 
This implies 
\begin{equation}
\label{eq:correlation_noise2}
\rho^{\prime} \left(b_{k}\right)=\lambda \times \rho\left(b_{k}\right)
\end{equation}
where,   
\begin{equation}
\label{eq:correlation_noise3}
\lambda = \frac{\sqrt{\sum_{n=0}^{N-1}\left(P_{n} -\bar{P}\right)^{2}}}{\sqrt{{\sum_{n=0}^{N-1}\left(P_{n} -\bar{P}\right)^{2}}+{\sum_{n=0}^{N-1} R_{n}^{2}}}}
\end{equation}


Fig.~\ref{fig:CorrelationBitByBit} shows that the modified correlation coefficient \(\rho ^{\prime}(b_{k}) \) decreases as the additive noise increases based on (\ref{eq:correlation_noise2}) and   (\ref{eq:correlation_noise3}). 

With this model, a threshold evaluation of the CPA's success is possible. 
Multiple experiments with additive noise are performed to investigate the influence of the noise on the correlation coefficients.
A comparison of the correlation with different amounts of additive noise is shown in Table~\ref{table:Comparing_results} and illustrated in Fig.~\ref{fig:Noise_compare}.
The results show how an increasing noise level impacts the correlation coefficient, ultimately making the correct candidate indistinguishable from other candidates.
For too low SNR, the CPA cannot successfully reveal the weights from the AI accelerator. 

Furthermore, multiple simulations are performed to investigate the impact of a noisy environment on the CPA.
Success is measured by the number of revealed secret \(PE\) parameters (weights).
Choosing random numbers for all inputs of the TPU leads to a success for 8 out of 9 parameters.
Tuning the input by feeding \(PE_{11}\) with zeroes increases the impact of other \(PEs\) on total power consumption.
This can be considered as a chosen plain text attack.
By utilizing this technique, the adversary can reveal all 9 hidden TPU parameters successfully.
When attacking a single \textit{PE}, a proportion of the power trace is always generated by the operations performed by circuitry other than the targeted \textit{PE}.
Although input tuning minimises the impact of certain \textit{PEs} on the power trace, the proportion on other circuitry cannot be completely eliminated.
If the impact of the non-targeted circuitry is defined as noise, our observations can provide suggestions for an architectural approach to overcome the leakage without dedicated noise-producing circuitry.
This enables a systematic exploration of the CPA limitations from an ESL point of view, i.e the design space exploration for security.

%%Any real hardware accelerator would have hundreds of \textit{PEs} performing calculations in parallel. Therefore, we can model the proportion of the power consumption from these \textit{PEs} as noise. Since adversary cannot extract the power consumption of one particular PE, and has to take advantage of input tuning to miniminze the proportion of the power consumption of other non-target \textit{PEs}. If we overcome the issues of input tuning, and \textit{PEs} executing their operations at slightly different points in time, we could suggest a CPA resistant architecture of a systolic array-based AI accelerator.
\begin{comment}

\begin{table}[t]
\caption{Impact of noise on revealing \textit{PE11s}  weight}
\resizebox{0.95\hsize}{!}{
\label{table:Comparing_results}
\centering
\begin{tabular}{ccc}
\toprule
\textbf{SNR} & \textbf{Correlation Coefficient} & \textbf{Attack Outcome} \\
\midrule
\textbf{10} & 0.755 & Successful \\
%\textbf{9} & 0.739 & Successful \\
\textbf{8} & 0.722 & Successful \\
%\textbf{7} & 0.706 & Successful \\
\textbf{6} & 0.678 & Successful \\
%\textbf{5} & 0.593 & Successful \\
\textbf{4} & 0.561 & Successful \\
\textbf{3.5} & 0.444 & Successful \\
\textbf{3} & 0.396 & Not Successful \\
\textbf{2.5} & 0.445 & Not Successful \\
\textbf{2} & 0.299 & Not Successful \\
\textbf{1.5} & 0.284 & Not Successful \\
\bottomrule
\end{tabular}}
\end{table}

\end{comment}

\subsection{Impact of Additive Noise on Template Attacks}
Several experiments are conducted to study the impact of additive noise on template attacks, where, both the profiling and attack traces are affected. 
Similar to the CPA evaluation, SNR is used to describe the magnitude of the noise.
The experiments show that recovering the weights of the leftmost and middle columns of \(PEs\) remains as easy as without noise.
By increasing the impact of noise i.e., decreasing SNR ranging between 2.5 and 2.0 using steps of 0.1, we demonstrate that template attacks on the leftmost and middle columns of \(PEs\) are successful with as little as 10 attack traces, as outlined in Table~\ref{table:TA_Noise_Results}.
It should be noted that we use the same ten attack traces to recover all three weights per column simultaneously (through applying an individual template for each of the weights).
The rightmost column of the \(PEs\) could also be attacked successfully with 10 attack traces, but here, different power traces are required for each \(PEs\) (with an individual template), denoted by * in Table~\ref{table:TA_Noise_Results}. 

Template attacks are still applicable for much lower SNR values, i.e., the template attacks are much less affected by noise if the same noise level is present during the profiling phase as well as the attack phase, as expected.
Template attacks therefore pose a serious threat to implementations even if the traces are very noisy.
By taking advantage of input tuning (as a chosen plaintext attack), an adversary could theoretically attack systolic arrays of any size and reveal secret parameters from a single \(PE\).

\todo[inline]{You somewhat lost me w/ regard to the leftmost, middle, and rightmost columns. For the first two, noise does not play a role, but for the last it somewhat does, requiring different power traces. Why? Also: Too low SNR is bad (obviously), but "much lower" SNR still works. Why? Then suddenly a twist, that if (the same?) noise is present during profiling and attack, template attacks work better. I also think this makes perfect sense, but never the less the reader might expect a short explanation, why that is so. As I see, this is outlined later in VIIa/b, so a forward reference like "we will detail this in Sections X/Y" might be enough.}

%\begin{table}[t]
%\caption{Impact of noise on revealing weights through template attacks}
%\resizebox{0.85\hsize}{!}{
%\label{table:TA_Noise_Results}
%\centering
%\begin{tabular}{cccc}
%\toprule
%\multirow{2}{*}{\textbf{SNR}} & \multicolumn{3}{c}{\textbf{Attack traces for successful recovery}} \\
%& \textbf{Column 1} & \textbf{Column 2} & \textbf{Column 3} \\
%\midrule
%\textbf{2.5} & 10 & 10 & 10* \\
%\textbf{2.4} & 10 & 10 & 10* \\
%\textbf{2.3} & 10 & 10 & 10* \\
%\textbf{2.2} & 10 & 10 & 10* \\
%\textbf{2.1} & 10 & 10 & 10* \\
%\textbf{2.0} & 10 & 10 & 10* \\
%\bottomrule
%\end{tabular}}
%\end{table}

It should be noted that this work analyses the impact of additive noise on CPA and Template attack, and it does not suggest the hardware realization of additive noise as a countermeasure.




%Since the impact of noise on the template attack should be less severe compared to the CPA \cite{TemplateAttacks}, successful attacks should be possible with even lower SNR values. 

%In order to investigate how much points of interest are sufficient for a successful attack, several experiments have been conducted.

%Even with noisy traces, specifying three points of interest proved to be sufficient.


==> 08-Model_verification_old.tex <==
\section{Model Verification}

\begin{figure}[t]
\includegraphics[width=\hsize, trim={0.5cm 1cm 4cm 0.5cm}]{figures/Systolic-array-3x3.pdf}
\centering
\caption{Systolic Array Implemented for Verification}
\label{fig:Diagram:SystolicArray}
\end{figure}

To verify the input-dependent power model utilized in our SystemC simulation of a systolic array, a gate-level power estimation of equivalent hardware units was performed. As discussed before, the power estimation model is suitable to analyse the behaviour of real hardware implementation, when the relative dynamic power consumption is considered (i.e. simulation of side-channel attacks). Naturally, raising the abstraction level brings an accuracy drop. Nevertheless, a comparison of the proposed SystemC-based model with a real hardware implementation can be performed. Therefore, a Verilog RTL implementation of a single PE, as well as the whole systolic array, was created. To make the power estimation of the real hardware even more realistic, we synthesized the designs using Synopsys DesignCompiler with the 14nm educational technology library from Synopsys to generate a gate-level netlist.



It was previously shown \textcolor{red}{[cite something about power estimation at gate-level]}, that a time-based power estimation at this abstraction level comes really close to post-silicon measurements. One of the tools used in the industry to perform the described tasks is Synopsys PrimePower. A pre-defined test-bench was used to stimulate the netlist and gather a value-change dump (VCD). In a addition to the 14nm technology library, the VCD was used to create a power trace from PrimePower in a time-based power analysis. These power traces are considered to be a noise-free reference trace of the real hardware. 


Repeating the simulations with an equivalent test-bench for our SystemC model, we can create traces that are comparable with cycle-accurate precision. The expectation is that the models' scaling behaviour behaves in a similar way as when we perform attacks. This means, we expect the two trace sets to correlate the most when modelling smaller pieces or hardware. The first comparison of just a single PE confirms this assumption. Using the same random inputs in both simulations (up to 20 000 traces), we observe a strong positive correlation between the traces, as seen in Fig.~\ref{fig:Traces-Correlation}. The value of up to 0.65 confirms that the proposed model follows the power consumption tendency of a real hardware implementation. To exclude false positives, the same simulation with two different sets of random inputs are repeated. Here, we observe a correlation coefficient close to 0, as shown in the upper right graph in Fig. \ref{fig:Traces-Correlation}.

\begin{figure}[t]
\includegraphics[width=\hsize]{figures/trace-verification.pdf}
\centering
\caption{Correlation coefficient between trace sets}
\label{fig:Traces-Correlation}
\end{figure}


The design of the whole systolic array is more complex. A test-bench with full coverage of all possible input/weight combinations for all PEs would produce an enormous amount of traces. Therefore, we fixed the weights in the PEs and stimulated the systolic array by 20\,000 random input samples.
An equivalent test-bench is implemented in SystemC to produce comparable traces. When evaluating the correlation coefficient between the two sets, we observe a stable correlation coefficient of 0.3. 
While at first sight this indicates a much worse correlation, the model complexity at netlist level needs to be taken into consideration. Hence, the measured value clearly signals correlation of both traces. This is confirmed by the counter-experiment:
%This is obviously a smaller value compared to the single PE, but considering the complexity of the implementation at netlist level, it can be said that the traces correlate. 
simulations with sets of different random inputs values lead to a correlation coefficient close to 0, therefore we exclude the possibility of a false-positive correlation. 
As a conclusion, it can be said that the proposed power estimation model follows the same trends as state-of-the-art netlist-level estimation. The value decrease of the correlation coefficient can be explained by the non-linearity caused by the missing estimation in the power-consumption behaviour of the clock-network of our systolic array. \textbf{\color{red}Is this only an assumption or do we have proof? "Can be explained" always sounds fishy to me, like some sort of magic handwaving ...}
